Quantum codes for asymmetric channels: ZZZY surface codes

We introduce surface ZZZY codes, a novel family of quantum error-correcting codes designed for asymmetric channels. Derived from standard surface codes through tailored modification of generators, ZZZY codes can be decoded by the minimum weight perfect matching (MWPM) algorithm with a suitable pre-processing phase. The resulting decoder exploits the information provided by the modified generators without introducing additional complexity. ZZZY codes demonstrate a significant performance advantage over surface codes when increasing the channel asymmetry, while maintaining the same correction capability over depolarizing channel.

==> Files/plot_varA41.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=0.001,
xmax=1000,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={A},
ymode=log,
ymin=1.22458148601383e-05,
ymax=6.56401699215876e-05,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={$\rho{}_\text{l}$},
axis background/.style={fill=white},
title style={font=\bfseries},
title={$\rho{}_\text{l}\text{ [[41,1,5]] and [[41,1,5]] varying A}$},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, dashed]
  table[row sep=crcr]{%
0.001	5.06825045799662e-05\\
0.00148735210729351	5.06537532266031e-05\\
0.00221221629107045	5.06110490352926e-05\\
0.00329034456231267	5.05476635621463e-05\\
0.00489390091847749	5.04536753335736e-05\\
0.00727895384398315	5.03145167519819e-05\\
0.0108263673387405	5.01089347333509e-05\\
0.0161026202756094	4.98062203950244e-05\\
0.0239502661998749	4.9362648684509e-05\\
0.0356224789026244	4.87173532398511e-05\\
0.0529831690628371	4.77885662448492e-05\\
0.0788046281566991	4.6472631951539e-05\\
0.117210229753348	4.46508378519032e-05\\
0.174332882219999	4.2212741422703e-05\\
0.259294379740467	3.91070079963699e-05\\
0.385662042116347	3.54247434299458e-05\\
0.573615251044868	3.14940817332936e-05\\
0.853167852417281	2.7915917270147e-05\\
1.26896100316792	2.54404674852486e-05\\
1.8873918221351	2.46616615269426e-05\\
2.80721620394118	2.56996823522697e-05\\
4.1753189365604	2.8136395605605e-05\\
6.21016941891562	3.12646294287608e-05\\
9.23670857187387	3.44275403462311e-05\\
13.7382379588326	3.72111244774844e-05\\
20.4335971785694	3.94514869539262e-05\\
30.3919538231319	4.11508394364395e-05\\
45.2035365636024	4.23896904562965e-05\\
67.2335753649934	4.32691214291697e-05\\
100	4.38823656180503e-05\\
1000	4.50632108171941e-05\\
};
\addlegendentry{[[41,1,5]]}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
0.001	4.44683599976396e-05\\
0.00148735210729351	4.44502863446513e-05\\
0.00221221629107045	4.44234366534041e-05\\
0.00329034456231267	4.43835727999304e-05\\
0.00489390091847749	4.43244380562264e-05\\
0.00727895384398315	4.42368294423572e-05\\
0.0108263673387405	4.41072844927978e-05\\
0.0161026202756094	4.39162717092328e-05\\
0.0239502661998749	4.36358059814059e-05\\
0.0356224789026244	4.32265456687697e-05\\
0.0529831690628371	4.26347896861626e-05\\
0.0788046281566991	4.17905862768708e-05\\
0.117210229753348	4.06096396639568e-05\\
0.174332882219999	3.90038812451971e-05\\
0.259294379740467	3.69074423891323e-05\\
0.385662042116347	3.43227880534387e-05\\
0.573615251044868	3.13793880530473e-05\\
0.853167852417281	2.83712079931391e-05\\
1.26896100316792	2.57172287072679e-05\\
1.8873918221351	2.38172624077896e-05\\
2.80721620394118	2.28710237596207e-05\\
4.1753189365604	2.27974244024227e-05\\
6.21016941891562	2.33163853446003e-05\\
9.23670857187387	2.41091574654449e-05\\
13.7382379588326	2.49349646370691e-05\\
20.4335971785694	2.56619517099157e-05\\
30.3919538231319	2.62435534906239e-05\\
45.2035365636024	2.66819675450479e-05\\
67.2335753649934	2.69999870379253e-05\\
100	2.72249184363479e-05\\
1000	2.76650425509075e-05\\
};
\addlegendentry{[[41,1,5]] XZZX}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
0.001	6.56401699215876e-05\\
0.00148735210729351	6.5602911837842e-05\\
0.00221221629107045	6.55475726323647e-05\\
0.00329034456231267	6.54654330586238e-05\\
0.00489390091847749	6.53436360545239e-05\\
0.00727895384398315	6.51633036469322e-05\\
0.0108263673387405	6.48968940422532e-05\\
0.0161026202756094	6.45046113142485e-05\\
0.0239502661998749	6.39297908792595e-05\\
0.0356224789026244	6.30935522672674e-05\\
0.0529831690628371	6.18899231630398e-05\\
0.0788046281566991	6.01845543809742e-05\\
0.117210229753348	5.78235592499287e-05\\
0.174332882219999	5.46637187233898e-05\\
0.259294379740467	5.06383231694814e-05\\
0.385662042116347	4.58651118819007e-05\\
0.573615251044868	4.07688091370711e-05\\
0.853167852417281	3.61274595720385e-05\\
1.26896100316792	3.29126426831792e-05\\
1.8873918221351	3.18937605849786e-05\\
2.80721620394118	3.32269547546855e-05\\
4.1753189365604	3.63714414891031e-05\\
6.21016941891562	4.0412180899003e-05\\
9.23670857187387	4.44991538748818e-05\\
13.7382379588326	4.80965286139745e-05\\
20.4335971785694	5.09920726501429e-05\\
30.3919538231319	5.31884634097377e-05\\
45.2035365636024	5.47896865899938e-05\\
67.2335753649934	5.59263650428742e-05\\
100	5.6718995459891e-05\\
1000	5.82452647878672e-05\\
};
\addlegendentry{[[25,1,5]]}

\addplot [color=mycolor4]
  table[row sep=crcr]{%
0.001	4.83587429906857e-05\\
0.00148735210729351	4.8348148712923e-05\\
0.00221221629107045	4.83324022445112e-05\\
0.00329034456231267	4.83090059010388e-05\\
0.00489390091847749	4.82742607337482e-05\\
0.00727895384398315	4.82227003108938e-05\\
0.0108263673387405	4.81462714865587e-05\\
0.0161026202756094	4.80331658329023e-05\\
0.0239502661998749	4.78661893444467e-05\\
0.0356224789026244	4.76205675367827e-05\\
0.0529831690628371	4.72611625887147e-05\\
0.0788046281566991	4.67393163961648e-05\\
0.117210229753348	4.59900754942314e-05\\
0.174332882219999	4.49315811713861e-05\\
0.259294379740467	4.34699551236604e-05\\
0.385662042116347	4.15144489700507e-05\\
0.573615251044868	3.90068162677647e-05\\
0.853167852417281	3.59621103494659e-05\\
1.26896100316792	3.25039512882466e-05\\
1.8873918221351	2.88650557885293e-05\\
2.80721620394118	2.53341538523219e-05\\
4.1753189365604	2.21690450059255e-05\\
6.21016941891562	1.95269708994584e-05\\
9.23670857187387	1.74484507191016e-05\\
13.7382379588326	1.58870255978419e-05\\
20.4335971785694	1.47533822772054e-05\\
30.3919538231319	1.39500711936327e-05\\
45.2035365636024	1.3390365769975e-05\\
67.2335753649934	1.30048750737257e-05\\
100	1.27414494085985e-05\\
1000	1.22458148601383e-05\\
};
\addlegendentry{[[25,1,5]] XZZX}

\end{axis}
\end{tikzpicture}%
